Finger Search in Grammar-Compressed Strings

Grammar-based compression, where one replaces a long string by a small context-free grammar that generates the string, is a simple and powerful paradigm that captures many popular compression schemes. Given a grammar, the random access problem is to compactly represent the grammar while supporting random access, that is, given a position in the original uncompressed string report the character at that position. In this paper we study the random access problem with the finger search property, that is, the time for a random access query should depend on the distance between a specified index $f$, called the \emph{finger}, and the query index $i$. We consider both a static variant, where we first place a finger and subsequently access indices near the finger efficiently, and a dynamic variant where also moving the finger such that the time depends on the distance moved is supported. Let $n$ be the size the grammar, and let $N$ be the size of the string. For the static variant we give a linear space representation that supports placing the finger in $O(\log N)$ time and subsequently accessing in $O(\log D)$ time, where $D$ is the distance between the finger and the accessed index. For the dynamic variant we give a linear space representation that supports placing the finger in $O(\log N)$ time and accessing and moving the finger in $O(\log D + \log \log N)$ time. Compared to the best linear space solution to random access, we improve a $O(\log N)$ query bound to $O(\log D)$ for the static variant and to $O(\log D + \log \log N)$ for the dynamic variant, while maintaining linear space. As an application of our results we obtain an improved solution to the longest common extension problem in grammar compressed strings. To obtain our results, we introduce several new techniques of independent interest, including a novel van Emde Boas style decomposition of grammars.

==> constanttime.tex <==
%!TEX root = paper.tex

\section{Constant Time Random Access and LCE}

In this section we describe a data structure that supports constant time random access and LCE queries in an SLP. As shown in the following lemma, any SLP can be modified to have certain useful properties.

\begin{lemma}[Gawrychowski~\cite{gawrychowski2012faster}]\label{lem:rest}
Let $\str$ be a string of length $N$ compressed into an SLP $\slp$ of size $n$. We can choose an arbitrary $\chunk$ and modify $\slp$ in $O(N)$ time adding $O(n)$ new variables such that we can write $\str$ as $\str=\str(v_1)\circ \ldots \circ \str(v_m)$ with $m=\Theta(N/\chunk)$ and $N_{v_i}\leq \chunk$. Among the nodes $v_1,\ldots, v_m$ there are $d=O(n)$ distinct nodes, $v_1^*,\ldots,v_{d}^*$. We will refer to the substrings generated by $v_1,\ldots, v_m$ as \textit{blocks} and $v_1^*,\ldots,v_{d}^*$ as \textit{basic blocks}. Furthermore, for any substring $\str[i,j]$ of length $\chunk$ we can find $O(1)$ blocks to cover it, i.e., $\str[i,j]\in \str(v_1)\circ \ldots \circ \str(v_k)$ and $k=O(1)$.
\end{lemma}

The last property mentioned in the lemma is not explicitly shown in \cite{gawrychowski2012faster} but is crucial to our data structure, so for completeness we include a full proof. %in Appendix~\ref{app:lemma5}. 
Before the proof we introduce some terminology. Let $p=v_1,v_2,\ldots,v_k$ be a path in a forest $F$ such that $v_1$ is an ancestor of $v_k$. The \textit{left forest} of $p$ is composed of the subtrees $F(\leftc(v_i))$, where $1\leq i < k$ and $\leftc(v_i)$ is not on $p$. The \textit{right forest} of $p$ is defined similarly.\\

%For the proof we will describe an algorithm that transforms the SLP and show that the resulting SLP obeys the specifics of the lemma. On a high level, the algorithm selects all the nodes that generate strings of size $\Theta(\ell)$. This partitions $\str$ into a substrings where some are covered by the selected nodes and some are not. Suppose for simplicity that a substring $\str[i,j]$ that is not covered by a selected node has a substring of size $\Theta(\ell)$ on its left and on its right. We then use the path going from the selected node on the left to the selected node on the right to construct new grammars generating strings of length $O(\ell)$ that generate $\str[i,j]$.

\begin{proof}
First we show the algorithm for modifying the SLP and then we prove that the properties of the resulting SLP follow from the modification.

Let $\mathcal{B}$ be the set of nodes that generate strings of length greater than $\frac 1 2 \chunk$ and whose children generate strings of length less than or equal to $\frac 1 2 \chunk$. The nodes in $\mathcal{B}$ generate strings of length at most $\chunk$. Let $u',v'$ be an occurrence of $u,v\in \mathcal{B}$ in the parse tree of $\slp$ such that $u'$ is to the left of $v'$ and no other node from $\mathcal{B}$ occurs in the right forest of the path from $v'$ to $\nca(v',u')$ or in the left forest of the path from $u'$ to $\nca(v',u')$. For all such pairs $u',v'$, the forest $F_l$ contains the path from $u'$ to $\nca(u',v')$ and the forest $F_r$  contains the path from $v'$ to $\nca(u',v')$.

The two forests are labelled as follows. In $F_l$, if there is an edge $\{\leftc(v),v\}$ then we assign it the primary label $p(\{\leftc(v),v\})=\rightc(v)$ and secondary label $s(\{\leftc(v),v\})=\epsilon$. Labels for $F_r$ are defined conversely: If $\{\leftc(v),v\}$ is an edge then $p(\{\leftc(v),v\})=\epsilon$ and $s(\{\leftc(v),v\})=\rightc(v)$, if $\{\rightc(v),v\}$ is an edge then $p(\{\rightc(v),v\})=\leftc(v)$ and $s(\{\rightc(v),v\})=\epsilon$.

The size of $F_l$ and $F_r$ is $O(n)$. We prove this by arguing that a node only occurs X times in $F_l$ (and $F_r$). Let $v$ be a node in $F_l$. There can be at most two paths ending in $v$, because $v$ can only be the nearest common ancestor of one specific pair of nodes in $\mathcal{B}$, so $v$ occurs at most twice as a leaf in $F_l$. The node $v$ also occurs at most twice as an internal node in $F_l$. Let $w$ be a node in $\slp(v)$ that is also in $\mathcal{B}$. Let $u\in \mathcal{B}$ be any node occuring to the left of $w$ in the parse tree of $\slp$ without any other node from $\mathcal{B}$ occurring between them. If $u\in \slp(v)$ the the path from $w$ to $\nca(w,u)$ does not contain $v$. If $u\notin \slp(v)$, the path from $w$ to $v$ is the same for any $u$. Hence, $v$ occurs only once in $F_l$ for this case. Similarly, $v$ only occurs once in $F_l$ for the case where $u$ occurs to the right of $w$ in the parse tree without any other nodes from $\mathcal{B}$ between them.

Finding $\mathcal{B}$ takes $O(n)$ time. Finding the ancestors of each pair can be done in one pass of the parse tree by marking the highest node visited when going from one node in $\mathcal{B}$ to the next. One pass takes $O(N)$ time. The paths between nodes in $\mathcal{B}$ can be found in $O(N)$ time, so the construction of $F_l$ and $F_r$ can also be done in $O(N)$ time.

In the following we show how to use $F_l$ and $F_r$ to restructure the SLP. The algorithm proceeds in two rounds. First we compute $F_l$ and use it to restructure the SLP. Then we compute $F_r$ from the new SLP and use it to restructure the SLP once again.

Starting from the roots of $F_l$ (or $F_r$ in the second round of the algorithm), we partition the trees greedily into edge-disjoint clusters such that the length of the string generated by the concatenation of primary edge labels is at most $\chunk$ on any root to leaf path in a cluster. Consider a cluster rooted in $v\in F_l$ with leaves $v_1,\ldots,v_k$. For every root-to-leaf path in the cluster we build a tree over the primary and secondary labels on the path\footnote{To efficiently reuse subtrees when building the trees, they should be constructed from the root of $F_l$ and down. This ensures that there is a tree representing the edges of any path from the root to an internal node in $F_l$.}. Let $v_i$ be the current leaf and $t_p$ the root of the tree over primary labels and $t_s$ the root of tree over secondary labels. Replace $v_i$ by $v_i=t_s v t_p$ in $\slp$. In the second round, when we consider clusters in $F_r$, the node is replaced by $v_i=t_p v t_s$. The nodes of the trees rooted in $t_p$ and $t_s$ are the new nodes of the SLP. When a node in $\slp$ is replaced it generates the same string, so the resulting SLP also generates $\str$. %This concludes the proof of Lemma~\ref{lem:rest}.

Now we will show that $m=\Theta(N/\chunk)$ and that any substring of length $\chunk$ can be covered by $O(1)$ blocks. Consider two nodes $u,v$ in $\mathcal{B}$ that are next to each other in the parse tree of $\slp$. The nodes $u$ and $v$ represent blocks and the algorithm will try to construct new blocks to fill the gap between the strings generated by $u$ and $v$. To do this the algorithm groups nodes hanging to the right of the path from $u$ to $\nca(u,v)$ such that each group generates a string of length $\Theta(\chunk)$. There may however be some nodes on the path from $u$ to $\nca(u,v)$ that do not become part of a group, and therefore we might form one group with size $o(\chunk)$. This might also happen for the path from $v$ to $\nca(u,v)$. In other words, the gap between $u$ and $v$ is filled by some blocks of size $\Theta(\chunk)$ and at most two blocks of size $o(\chunk)$. From this it follows that $m=\Theta(N/\chunk)$ and any substring of length $O(\chunk)$ can be covered by $O(1)$ blocks.
% \begin{itemize}
% 	\item We will show that $m=\Theta(N/\chunk)$ and that any substring of length $\chunk$ can be covered by $O(1)$ blocks
% 	\item Consider two nodes $u,v$ in $\mathcal{B}$ that are next to eachother in the parse tree of $\slp$. 
% 	\item The nodes $u$ and $v$ represent blocks and the algorithm will try to construct new blocks to fill the gap between the strings generated by $u$ and $v$
% 	\item To do this the algorithm groups nodes hanging to the right of the path from $u$ to $\nca(u,v)$ such that each group generates a string of length $\Theta(\chunk)$
% 	\item There may however be some nodes left on the path from $u$ to $\nca(u,v)$ that do not become part of a group, and therefore we might form a group with size $o(\chunk)$
% 	\item This might also happen for the path from $v$ to $\nca(u,v)$
% 	\item In other words, the gap between $u$ and $v$ is filled by some blocks of size $\Theta(\chunk)$ and at most two blocks of size $o(\chunk)$ and this yields the properties stated in the lemma
% \end{itemize}
\qed
\end{proof}


%\begin{itemize}
%	\item We will refer to the substrings generated by $v_1,\ldots, v_m$ as \textit{blocks} and $v_1^*,\ldots,v_{d}^*$ as \textit{basic blocks} 
%	\item From the construction of Lemma~\ref{lem:rest} it also follows that for any substring of \str of length $\chunk$ we can find $O(1)$ blocks to cover it (needs proof?)
%\end{itemize}

% \begin{itemize}
% 	\item Overall idea
% 	\item After applying the construction from the above lemma we have that position $i$ is guaranteed to be in one of a constant number of blocks of size $\chunk$
% 	\item Our first idea is to explicitly store the strings generated by all basic blocks, and then split \str into substrings of size $\chunk$ and store references from these to the blocks covering them
% 	\item Next, we extend this idea to have multiple layers where only substrings of basic blocks on the last layer are stored
% \end{itemize}
\subsection{Random Access}

The general idea of our data structure is to explicitly store the strings generated by all basic blocks, and then split \str into substrings of size $\chunk$ and store references from these to the blocks covering them. When we want to access a position $i$ we find the substring of length $\chunk$ and the appertaining blocks that contains $i$. Next, we extend this idea to have multiple layers where only substrings of basic blocks on the deepest layer are stored.

\subsubsection{Basic data structure}
We apply the construction of Lemma~\ref{lem:rest} to $\slp$ and store the string generated by each basic block and its length. For every substring $\str[j\chunk+1,j\chunk+\chunk]$, $j=0\ldots\frac N \chunk-1$, we store a list of block roots $v_1,\ldots, v_k$ such that $\str[j\chunk,j\chunk+\chunk]$ is a substring of $\str(v_1)\circ \ldots \circ \str(v_k)$. We also store the index in $\str(v_1)\circ \ldots \circ \str(v_k)$ where $\str[j\chunk,j\chunk+\chunk]$ occurs.

An $\access(i)$ query is answered as follows. Let $\str[j\chunk,j\chunk+\chunk]$ be the length-$\chunk$ substring that contains position $i$. Let $s=\str(v_1)\circ \ldots \circ \str(v_k)$ be the blocks containing this substring and $p$ the position in $s$ where it begins. We want to return $s[p+i-j\chunk]$. To do so, we find the block root $v_r$ where $\sum_{l=1}^{r-1}N_{v_l}< p+i-j\chunk \leq \sum_{l=1}^{r}N_{v_l}$ and return $S(v_r)[p+i-j\chunk-\sum_{l=1}^{r-1}N_{v_l}]$.

The SLP resulting from applying Lemma~\ref{lem:rest} has $O(n)$ nodes. Storing the substrings generated by basic blocks require $O(n\chunk)$ space. For each of the $N/\chunk$ substrings of $\str$ we store a constant number of block roots, i.e., $k=O(1)$ for each substring. Hence, this requires $O(N/\chunk)$ space. In total our data structure uses $O(n\chunk+N/\chunk)$ space which is $O(\sqrt{nN})$ space when balancing the two terms.  Computing the appropriate length-$\chunk$ substring is by integer division and takes constant time and then we search $k=O(1)$ blocks until we have found the substring containing $\str[i]$. Thus, a query takes $O(1)$ time.

% \begin{itemize}
% 		\item Data structure:
% 		\item Apply the construction of Lemma~\ref{lem:rest} to $\slp$
% 		\item We store the string generated by each basic block and its length
% 		\item For every substring $\str[j\chunk+1,j\chunk+\chunk]$, $j=0..\frac N \chunk-1$, store a list of block roots $v_1,\ldots, v_k$ such that $\str[j\chunk,j\chunk+\chunk]$ is a substring of $\str(v_1)\circ \ldots \circ \str(v_k)$ 
% 		\item We also store the index in $\str(v_1)\circ \ldots \circ \str(v_k)$ where $\str[j\chunk,j\chunk+\chunk]$ occurs 
% 		\item Query:
% 		\item An $\access(i)$ query is answered as follows
% 		\item We compute which length-$\chunk$ substring that contains $i$, let $\str[j\chunk,j\chunk+\chunk]$ be this string
% 		\item Let $s=\str(v_1)\circ \ldots \circ \str(v_k)$ be the chunks containing this substring and $p$ the position in $s$ where the substring begins
% 		\item We want to return $s[p+i-j\chunk]$
% 		\item To do so, we find the node $v_r$ where $\sum_{l=1}^{r-1}|S(v_l)|< p+i-j\chunk \leq \sum_{l=1}^{r}|S(v_l)|$ and return $S(v_r)[p+i-j\chunk-\sum_{l=1}^{r-1}|S(v_l)|]$
% 		\item Analysis
% 		\item Space:
% 		\item The SLP resulting from applying Lemma~\ref{lem:rest} has $O(n)$ nodes
% 		\item We store the string generated by $O(n)$ nodes of size at most $\chunk$, totalling $O(n\chunk)$ space
% 		\item Storing the length of the strings generated by nodes requires a total of $O(n)$ space
% 		\item For each of the $N/\chunk$ substrings of $\str$ we a store a list of $k=O(1)$ nodes since Lemma~\ref{lem:rest} allows us to find $O(1)$ nodes such that concatenation of their strings contains a substring of length $\chunk$
% 		\item Hence, this requires $O(N/\chunk)$ space
% 		\item In total our data structure uses $O(n\chunk+N/\chunk)$ space which is $O(\sqrt{nN})$ space when balancing the two terms
% 		\item A query takes $O(1)$ time. 
% 		\item Finding the appropriate length-$\chunk$ substring clearly takes constant time and then we search $k=O(1)$ blocks until we have found the substring containing $\str[i]$.
% 	\end{itemize}


\subsubsection{Extending to more layers}

We now show how to extend the basic data structure to multiple layers and hereby obtain the results of Thm~\ref{thm:ConstTimeRA}.

We select $k$ parameters $\chunk_1,\chunk_2,\ldots,\chunk_k$ where each $\chunk_i>5$. Suppose we are applying the construction for layer $i>1$. Let the roots of blocks created for layer $i-1$ be temporary leaves of the SLP. Apply the construction of Lemma~\ref{lem:rest} with parameter $\chunk_i$ to the SLP with temporary leaves. The following lemma gives a general bound on the number of blocks required to cover a string with length proportional to the size of a string generated by a block on some layer.

% \begin{itemize}
% 	\item Layering the construction of Lemma~\ref{lem:rest}
% 	\item Select $k$ parameters $\chunk_1,\chunk_2,\ldots,\chunk_k$ where each $\chunk_i>2$
% 	\item Suppose we are applying the construction for layer $i$
% 	\item Let the roots of the chunks created for layer $i-1$ be temporary leaves of the SLP and assign them size 1
% 	\item Apply the construction of Lemma~\ref{lem:rest} with parameter $\chunk_i$ to the SLP
% 	\item When creating layer $i$ we add a number of nodes linear in the size of the SLP after creating layer $i-1$, she size of the SLP resulting from applying Lemma~\ref{lem:rest} in layers as describe above is $O(
% 	2^kn)$
% 	\item An important property of Lemma~\ref{lem:rest} is generalized in the following lemma.
% \end{itemize}

\begin{lemma}\label{lem:generalBlock}
Consider a root $v$ of a block created in layer $i>1$. For any substring of $\str(v)$ of length $O(\prod_{j=1}^{i-1} \chunk_j)$ we can find $O(2^{i-1})$ blocks in layer $i-1$ to cover it.
\end{lemma}

\begin{proof}
The proof is by induction on $i$. A \textit{big block} on layer $i$ is a block of size $\Theta(\chunk_i)$ and a \textit{small block} is a block of size $o(\chunk_i)$. It is seen in the proof of Lemma~\ref{lem:rest} that there can be at most two small blocks between two big blocks. 

$i=2$: A big block spans at least $3$ blocks from layer 1 and at most two of these are small. Therefore a big block $v$ in layer $2$ generates a string of size $\frac{\chunk_1\chunk_2}{c_1}< N_v \leq \chunk_1\chunk_2$ for some constant $c_1>1$. Like on layer 1, two big blocks can be separated by at most two blocks of size $o(\chunk_1\chunk_2)$ so for any string of length $O(\chunk_1\chunk_2)$ we need at most $c_1+O(1)=O(1)$ blocks to cover it.

$i>2$: A big block $v$ in layer $i$ generates a string of size $\frac{\prod_{j=1}^i \chunk_j}{\prod_{j=1}^{i-1} c_j}< N_v \leq \prod_{j=1}^i \chunk_j$ where $c_1,\ldots,c_{i-1}$ are constants. Two big blocks are separated by at most two blocks of size $o(\chunk_i)$ so for any string of length $O(\prod_{j=1}^i \chunk_j)$ we need at most $\prod_{j=1}^{i-1} c_j+O(1)=O(2^{i-1})$ blocks to cover it.
% \begin{itemize}
% 	%\item We will prove by induction that at most two consecutive blocks in layer $i-1$ are of size $o(\prod_{j=1}^i \chunk_j)$ which implies the lemma.
% 	\item A \textit{big block} on layer $1$ is a block of size $\Theta(\chunk_1)$ and a \textit{small block} is a block of size $o(\chunk_1)$. Recall from Lemma~\ref{lem:rest} that there can be at most two small blocks between two big blocks. 
% 	\item \textit{Base case, $i=2$.}
% 	\item A big block spans at least $3$ blocks from layer 1 and at most two of these are small. Therefore a block $v$ in layer $2$ has size $\frac{\chunk_1\chunk_2}{c_1}<|v|\leq \chunk_1\chunk_2$ for some constant $c_1>1$.
% 	\item Like on layer 1, two big blocks can be separated by at most two blocks of size $o(\chunk_1\chunk_2)$ so for any string of length $O(\chunk_1\chunk_2)$ we need at most $c_1+O(1)=O(1)$ blocks to cover it.
% 	\item \textit{Induction, $i>2$.}
% 	\item A big block in layer $i$ has size $\frac{\prod_{j=1}^i \chunk_j}{\prod_{j=1}^{i-1} c_j}<|v|\leq \prod_{j=1}^i \chunk_j$ where $c_1,\ldots,c_{i-1}$ are constants
% 	\item Two big blocks are separated by at most two blocks of size $o(\prod_{j=1}^i \chunk_j)$ so for any string of length $O(\prod_{j=1}^i \chunk_j)$ we need at most $\prod_{j=1}^{i-1} c_j+O(1)=O(2^{i-1})$ blocks to cover it.
% \end{itemize}
\qed
\end{proof}

Our data structure consists of the layering of blocks as described above. For the deepest layer we explicitly store the strings generated by basic blocks. For every root $v_r$ of a basic block in layer $i$ we store a list of the blocks that cover every substring $\str(v_r)[j\chunk_{i-1},j\chunk_{i-1}+\chunk]$, $j=0\ldots\frac{N_{v_r}}{\chunk_{i}}-1$, as we did for the basic data structure.

To answer an $\access(i)$ query we start from the root of the SLP and find the block that contains position $i$ as described in the previous section. This is repeated from the root of the resulting basic block until we reach a block in the deepest layer.

% \begin{itemize}
% 	\item Start from the root of the SLP
% 	\item Find the chunk that contains $i$ as described in the previous section
% 	\item Repeat the process from the root of the chunk until we reach a chunk for which explicitly have stored the string
% \end{itemize}

When creating layer $i$ we add a number of nodes linear in the size of the SLP after creating layer $i-1$, so the size of the SLP resulting from applying Lemma~\ref{lem:rest} in layers is $O(2^kn)$. The substring generated by a basic block in layer $i$ is split into $\chunk_i/\chunk_{i-1}$ substrings for each of which we store a list of $O(2^{i-1})$ blocks (Lemma~\ref{lem:generalBlock}). There are $O(n)$ basic blocks in a layer, so for layer $i$ this uses $O(2^{i-1}n\chunk_i/\chunk_{i-1})$ space. For the top layer this uses $O(2^{k-1}N/\chunk_k)$ space and we use $O(n\chunk_1)$ space to explicitly store strings in the bottom layer. In total, the space usage of our data structure is $O(2^kn+ 2^{k-1}N/\chunk_k+ \sum_{i=2}^{k} 2^i n\chunk_i/\chunk_{i-1} + n\chunk_1)$. Choose $k$ to be some arbitrarily large constant and balance the terms and the space becomes $O(n^{1-\epsilon}N^{\epsilon})$ for any constant $\epsilon > 0$. In the query, we spend $O(1)$ time for each of the constant number of layers, hence $O(1)$ time in total. This proves Thm.~\ref{thm:ConstTimeRA}.

% \begin{itemize}
% 	\item When creating layer $i$ we add a number of nodes linear in the size of the SLP after creating layer $i-1$, so the size of the SLP resulting from applying Lemma~\ref{lem:rest} in layers is $O(2^kn)$.
% 	\item Explain the space used in each layer
% 	\item The space usage of our data structure is $O(2^kn+ n/\chunk_1+n\chunk_1/\chunk_2+\ldots +n\chunk_{k-1}/\chunk_k + n\chunk_k)$
% 	\item Choose $k$ to be some arbitrarily large constant and balance the terms and the space becomes $O(n^{1-\epsilon}N^{\epsilon})$ for some constant $\epsilon > 0$
% 	\item In the query, we spend $O(1)$ time for each layer, hence $O(1)$ time in total
% 	\item This concludes Theorem~\ref{thm:ConstTimeRA}
% \end{itemize}

\subsection{Longest Common Extensions}

We now extend our data structure to support LCE queries. 

We use \textit{difference covers} (see e.g.~\cite{DBLP:journals/ipl/ColbournL00}) to sample positions of a string. A difference cover modulo $\tau$ is a set of integers $D\subseteq\{0,1,\ldots,\tau-1\}$ such that for any $d\in[0,\tau-1]$, $D$ contains two elements separated by distance $d$ modulo $\tau$. To represent $\tau$ differences a difference cover has to have at least $\sqrt\tau$ elements. In our data structure we will use the difference cover $\{0,\ldots,\sqrt\tau-1\}\cup\{i\sqrt\tau \mid i=1\ldots\sqrt\tau\}$ of size $2\sqrt\tau -1$. It has the property that given a distance $d$, the two elements with distance $d$ modulo $\tau$ can be found in constant time.

%Suppose we have computed a difference cover for $\tau$. We split the string into $N/\tau$ substrings and for each substring we sample the positions determined by our difference cover. Suppose we are given two positions in the string that are not included in our sample. As a property of difference covers we can find two positions in the sample by shifting both positions by at most $\tau$.



% \begin{lemma}[Colbourn and Ling~\cite{DBLP:journals/ipl/ColbournL00}]
% For any $\tau$, a difference cover modulo $\tau$ of size at most $\sqrt{1.5\tau} + 6$ can be computed in $O(\sqrt \tau)$ time.
% \end{lemma}



%We will also use the following well-known result for LCE.

%\begin{lemma}\label{lem:LCE}
%Given a string $\str$ of size $N$, there is a data structure of size $O(N)$ which supports LCE queries in $O(1)$ time. 
%\end{lemma}

%To get Lemma~\ref{lem:LCE} we build the \textit{suffix tree}~\cite{mccreight1976space,ukkonen:on-line,farach,WeinerSTconstruction} of $\str$ and build a \textit{nearest common ancestor} (NCA) data structure with constant query time~\cite{harel1984fast,Bender:2000:LPR:646388.690192} for the tree. To answer a query in position $i$ and $j$, we find the leaves representing the suffixes starting in $i$ and $j$ and report the string depth of their nearest common ancestor in the suffix tree.

Moreover, recall that there is an LCE data structure using $O(N)$ space with query time $O(1)$. By using a \textit{sparse suffix tree}~\cite{kaerkkaeinen96sparse,bille2013sparse} we may create a restricted version of this data structure that is only capable of answering LCE queries for positions corresponding to suffixes in the sparse suffix tree. We will refer to this as a \textit{sparse LCE data structure}. Since we are only using the sparse suffix tree for LCE queries we do not have to keep the labels on the edges of the tree, the size of the sparse LCE data structure is linear in the number of suffixes in the tree.

\subsubsection{Basic data structure}

Similarly to the previous section, we will first describe a basic version of our data structure and then extend it to have multiple layers.

Assume we have computed a difference cover $D$ for $\tau=\chunk$ and denote by $D_i$ the set of integers where each element from $D$ is increased by $i\chunk$. Let $D^*=D\cup D_1\cup\ldots \cup D_{N/X}$ be the difference cover obtained by sampling positions from $D$ in each length-$\chunk$ substring of $\str$.

We store the sparse LCE data structure for the positions in $D^*$. We also build the random access data structure described in the previous section. We concatenate the strings generated by basic blocks, separated by $O(n)$ special characters not occurring elsewhere, and store an LCE data structure for this. 

% \begin{itemize}
% 	\item Compute a difference cover $D$ for $\tau=\chunk$
% 	\item Denote by $D_i$ the set of integers where each element from $D$ is increased by $i\chunk$
% 	\item Build the sparse suffix tree for the positions $D^*=D\cup D_1\cup\ldots \cup D_{N/X}$. $D^*$ is a difference cover of size $O(N/\sqrt \chunk)$ for $[0,N-1]$
% 	\item We do not label the edges of the suffix tree. In the nodes we store the string depth of prefixes of suffixes
% 	\item Build NCA data structure for the sparse suffix tree
% 	\item Apply Lemma~\ref{lem:rest} to the SLP
% 	\item For each basic block we build the data structure of Lemma~\ref{lem:LCE}
% 	\item Build the random access data structure described in the previous section
% \end{itemize}

To answer an $\lce(i,j)$ query we use our data structure as follows. If $i,j\in D^*$ the answer to the query is found with the sparse LCE data structure. If not, we first compute the smallest $i'>i$ and $j'>j$ such that $i',j'\in D^*$ and $i'-i=j'-j$. Using the random access data structure we find the blocks covering the strings $\str[i,i']$ and $\str[j,j']$. We then use the LCE data structure for the concatenated basic blocks to find the LCE of $i$ and $j$ in the blocks covering $\str[i,i']$ and $\str[j,j']$. The boundaries of the blocks may not be aligned, so if the end of one of the two current blocks is reached we continue the query from the beginning of the next block. This is repeated until we have either found that the LCE is less than $i'-i$ or greater than or equal to $i'-i$. In the first case, the final answer to the query is now known and we terminate. In the latter case, the query is continued in the sparse LCE data structure for the positions $i'$ and $j'$ and the final answer is $i'-i$ plus this answer.

% \begin{itemize}
% 	\item $\lce(i,j)$
% 	\item If $i,j\in D^*$ the answer to the query is the string depth of the NCA in the sparse suffix tree for the positions in $D^*$
% 	\item If not, then we proceed as follows
% 	\item We first compute the smallest $i'>i$ and $j'>j$ such that $i',j'\in D^*$ and $i'-i=j'-j$ (how?)
% 	\item Using our random access data structure we find the blocks covering the strings $\str[i,i']$ and $\str[j,j']$
% 	\item We first perform an LCE query in the blocks containing $i$ and $j$, say $v_i$ and $v_j$
% 	\item If the end of a one of the two blocks is reached in the query we continue the query from the beginning of the next block
% 	\item We continue doing this until we have either found that the LCE is less than $i'-i$ or we greater than or equal to $i'-i$
% 	\item In the first case, the answer is the LCE that we have just computed
% 	\item In the latter case, the query is continued in the sparse suffix tree for the positions $i'$ and $j'$
% \end{itemize}

The random access data structure uses $O(N/\chunk + n\chunk)$ space. The sparse LCE data structure has size $O(N/\sqrt \chunk)$. For each basic block we use $O(\chunk)$ space for an LCE data structure totalling to $O(n\chunk)$ space. In total, the basic data structure uses $O(N/\sqrt \chunk + n\chunk)$ space which is $O(n^{1/3}N^{2/3})$ when balancing the two terms.

% \begin{itemize}
% 	\item Space of data structure
% 	\item The sparse suffix tree has size $O(N/\sqrt \chunk)$
% 	\item For each basic block we use $O(\chunk)$ space (Lemma~\ref{lem:LCE}) totalling to $O(n\chunk)$ space
% 	\item The random access data structure uses $O(N/\chunk + n\chunk)$ space
% 	\item In total the basic data structure uses $O(N/\sqrt \chunk + n\chunk)$ space which is $O(n^{1/3}N^{2/3})$ when balancing the two terms
% \end{itemize}

We now argue that a query takes constant time. Computing $i'$ and $j'$ clearly takes constant time. Because $D,D_1,\ldots,D_{N/\chunk}$ are difference covers for $\chunk$ we have that $i'-i=j'-j\leq \chunk$. We know that we can find a constant number of blocks covering the substrings $\str[i,i']$ and $\str[j,j']$ and that we can answer LCE queries within blocks in constant time. Thus, we may compute the LCE in constant time for values less than or equal to $i'-i=j'-j\leq \chunk$. If the LCE is greater than this we use the sparse LCE data structure to decide the $\lce(i',j')$ value in constant time. In total, a query takes $O(1)$ time.

% \begin{itemize}
% 	\item We now argue that a query takes constant time
% 	\item Computing $i'$ and $j'$ clearly takes constant time
% 	\item Because $D,D_1,\ldots,D_{N/\chunk}$ is a difference cover for $\chunk$ we have that $i'-i=j'-j\leq \chunk$
% 	\item We know that we can find a constant number of blocks covering the substrings $\str[i,i']$ and $\str[j,j']$ and that we can answer LCE queries within blocks in constant time. Thus, we may compute the LCE in constant time for values less than or equal to $\chunk$
% 	\item If the LCE is greater than $\chunk$ we use the sparse suffix tree to decide the value in constant time
% 	\item In total a query takes $O(1)$ time
% \end{itemize}

\subsubsection{Extending to more layers}

First we build the random access data structure described in the previous section. Suppose we have computed difference covers for all parameters $\chunk_1,\ldots,\chunk_k$. For every basic block with root $v$ in layer $i$ we store a sparse LCE data structure for positions determined by the difference cover for $\chunk_i$ on every size-$\chunk_i$ substring of $\str(v)$. For all basic blocks in the deepest layer we store an LCE data structure. 

A query works as for the basic data structure but proceeds recursively on the layers until the positions are aligned on sampled positions or reaching the deepest level.

The space complexity analysis is similar to that of the random access data structure. We require $O(\chunk_i/\sqrt\chunk_{i-1})$ space to store the sparse LCE data structure for a basic block on layer $i$, hence the total space usage is 
$$
O(2^kn+ 2^{k-1}N/\chunk_k+ \sum_{i=2}^{k} 2^i n\chunk_i/\chunk_{i-1} + n\chunk_1)+
O(2^kn+ N/\sqrt\chunk_k+ \sum_{i=2}^k n\chunk_i/\sqrt\chunk_{i-1} + n\chunk_1)
$$
Choose $k$ to be some arbitrarily large constant and balance the terms and the space becomes $O(N^{\frac 1 2 +\epsilon}n^{\frac 1 2 - \epsilon})$. We spend constant time on each level and with $k=O(1)$ the resulting query time is $O(1)$. This concludes the proof of Thm.~\ref{thm:LCEres}$(i)$.

% \begin{itemize}
% 	\item Build random access data structure
% 	\item For all basic blocks in the deepest layer we store the LCE data structure of Lemma~\ref{lem:LCE}
% 	\item As with the basic data structure, we compute and store a difference cover for $\chunk_k$ and extend it to cover the entire string $\str$ and construct the sparse suffix tree for the suffixes in the difference cover
% 	\item Suppose we have a difference cover for each layer $i$ of size $O(\chunk_i/\sqrt\chunk_{i-1})$ constructed the same way as for the basic data structure
% 	\item For every basic block in layer $i$ we store the sparse suffix tree for the (relative) positions in the difference cover  
% \end{itemize}


% \begin{itemize}
% 	\item LCE space usage is $O(N^{1-\frac{2^i-1}{2^{i+1}-1}}n^{\frac{2^i-1}{2^{i+1}-1}})$.
% \end{itemize}
